Annealing approach to root-finding

The Newton-Raphson method is a fundamental root-finding technique with numerous applications in physics. In this study, we propose a parameterized variant of the Newton-Raphson method, inspired by principles from physics. Through analytical and empirical validation, we demonstrate that this novel approach offers increased robustness and faster convergence during root-finding iterations. Furthermore, we establish connections to the Adomian series method and provide a natural interpretation within a series framework. Remarkably, the introduced parameter, akin to a temperature variable, enables an annealing approach. This advancement sets the stage for a fresh exploration of numerical iterative root-finding methodologies.

==> table_1.tex <==
{
\begin{tabular}{p{5.5cm}|>{\centering\arraybackslash}p{0.9cm}>{\centering\arraybackslash}p{0.65cm}>{\centering\arraybackslash}p{0.65cm}>{\centering\arraybackslash}p{0.65cm}>{\centering\arraybackslash}p{0.65cm}|>{\centering\arraybackslash}p{0.9cm}>{\centering\arraybackslash}p{0.6cm}>{\centering\arraybackslash}p{0.6cm}>{\centering\arraybackslash}p{0.6cm}>{\centering\arraybackslash}p{0.6cm}|>{\centering\arraybackslash}p{0.9cm}>{\centering\arraybackslash}p{0.6cm}>{\centering\arraybackslash}p{0.5cm}>{\centering\arraybackslash}p{0.6cm}>{\centering\arraybackslash}p{0.6cm}}
    \hline
{\multirow{2}{*}{Functions}}  &   \multicolumn{5}{c|}{Iteration number} &   \multicolumn{5}{c|}{Convergence percentage} &   \multicolumn{5}{c}{Computation time}  \\
    \cline{2-16}
& {\footnotesize$\beta=$}$-1$ & $-0.5$ & $0$ & $0.5$ & $1$ & {\footnotesize$\beta=$}$-1$ & $-0.5$ & $0$ & $0.5$ & $1$ & {\footnotesize$\beta=$}$-1$ & $-0.5$ & $0$ & $0.5$ & $1$ \\
    \hline
{\footnotesize $f_1(x) = (x^2 - 1)(x^2 + 1)$}  & 18.4  & 15.7 & 11.3 & 11.0 & \bf{10.5} & 75  & 80 & \bf{100} & \hfil 91 & \hfil 90 & 1.50 & 1.29 & 1.0 & 0.92 & \bf{0.89}   \\
    \hline
{\footnotesize $f_2(x) = x^3 - 1$} & 15.5 & 13.3 & \hfil 9.1 & \hfil 9.1 & \hfil \bf{8.4} & 92 & 96 & \bf{100} & \hfil 99 & \hfil 99 & 1.55 & 1.35 & 1.0 & 0.94 & \bf{0.93} \\
\hline
{\footnotesize $f_3(x) = x^{12} - 1$} & 18.5 & 16.3 & 16.4 & 12.7 & \bf{11.5} & 44 & 56 & \hfil \bf{84} & \hfil 67 & \hfil 66 & 1.11 & 0.93 & 1.0 & 0.73 & \bf{0.67} \\
\hline
{\footnotesize $f_4(x) = (x^2 - 4)(x + 1.5)(x - 0.5)$} & 12.6 & 10.4 & \hfil 8.0 & \hfil 7.4 & \hfil \bf{6.4} & 98 & 97 & \bf{100} & \bf{100} & \bf{100} & 1.50 & 1.27 & 1.0 & 0.89 & \bf{0.79} \\
\hline
{\footnotesize $f_5(x) =(x+2)(x+1.5)^2 (x-0.5)(x-2)$} & 12.1 & \bf{10.3} & 28.9 & 25.6 & 22.2 & 42 & 43 & \hfil 96 & \hfil \bf{99} & \hfil \bf{99} & 0.42 & \bf{0.35} & 1.0 & 0.85 & 0.76 \\
\hline
{\footnotesize $f_6(x) = \sin(x)$} & \hfil 9.7 & \hfil 7.7 & \hfil 6.6 & \hfil 6.0 & \hfil \bf{5.5} & 87 & 84 & \bf{100} & \hfil 95 & 
 \hfil 92 & 1.42 & 1.09 & 1.0 & 0.87 & \bf{0.82} \\
\hline
{\footnotesize $f_7(x) = (x - 1)^3 + 4(x-1)^2 - 10$} & 17.9 & 14.5 & \hfil 9.7 & \hfil 9.1 & \hfil \bf{8.4} & 97 & 97 & \bf{100} & \bf{100} & \bf{100} & 1.74 & 1.44 & 1.0 & 0.92 & \bf{0.83} \\
\hline
{\footnotesize $f_8(x) = \sin(x-14/10)^2 - (x - 14/10)^2 + 1$} & 11.3 & \hfil 9.4 & \hfil 8.9 & \hfil 7.5 & \hfil \bf{6.5} & 60 & 59 & \hfil \bf{71} & \hfil 64 & \hfil 64 & 1.25 & 1.04 & 1.0 & 0.86 & \bf{0.76} \\
\hline
{\footnotesize $f_9(x) = x^2 - e^x - 3x + 2$} & \hfil 8.1 & \hfil 7.1 & \hfil 6.2 & \hfil 5.8 & \hfil \bf{5.0} & 97 & 97 & \bf{100} & \hfil 99 & \hfil 98 & 1.20 & 1.13 & 1.0 & 0.93 & \bf{0.79} \\
\hline
{\footnotesize $f_{10}(x) = \cos(x-3/4) - x + 3/4$} & 10.8 & \hfil 8.8 & \hfil 8.6 & \hfil 7.1 & \hfil \bf{6.3} & 61 & 63 & \bf{93} & \hfil 75 & \hfil 72 & 1.23 & 0.97 & 1.0 & 0.8 & \bf{0.72} \\
\hline 
{\footnotesize $f_{11}(x) = (x + 1)^3 - 1$} & 15.1 & 12.7 & \hfil 9.0 & \hfil 8.9 & \hfil \bf{8.1} & 93 & 96 & \bf{100} & \hfil 99 & \hfil 99 & 1.50 & 1.29 & 1.0 & 0.96 & \bf{0.85} \\
\hline
{\footnotesize $f_{12}(x) = (x-2)^3 - 10$} & 17.5 & 14.7 & \hfil 9.3 & \hfil 9.8 & \hfil \bf{8.9} & 87 & 92 & \bf{100} & \hfil 97 & \hfil 98 & 1.84 & 1.54 & 1.0 & 1.01 & \bf{0.96} \\
\hline
{\footnotesize $f_{13}(x) = (x+5/4) e^{(x+5/4)^2} - \sin(x+5/4)^2 + 3\cos(x+5/4) + 5$} & 17.0 & 13.2 & 11.6 & \hfil 9.7 & \hfil \bf{9.4} & 55 & 60 & \bf{96} & \hfil 82 & \hfil 80 & 1.46 & 1.12 & 1.0 & 0.81 & \bf{0.80} \\
\hline
{\footnotesize $f_{14}(x) = x + \sin(2/x)  x^2$} & 15.5 & 13.5 & 10.9 & \hfil \bf{9.5} & 10.3 & 35 & 57 & \bf{99} & \hfil 88 & \hfil 74 & 1.41 & 1.22 & 1.0 & \bf{0.86} & 1.08 \\
\hline
\end{tabular}
}



 %& \multicolumn{5}{c}{Mean iterations/point} & \multicolumn{5}{c}{Non 
 %convergent (\%)} &\multicolumn{5}{c}{Time/point (relative to $\beta = 0$)} \\    
% & \multicolumn{5}{c}{$\beta$} & \multicolumn{5}{c}{$\beta$} &\multicolumn{5}{c}{$\beta$} \\
% \hline
% & -1 & -0.5 & 0 & 0.5 & 1 &-1 & -0.5 & 0 & 0.5 & 1 &-1 & -0.5 & 0 & 0.5 & 1 \\
%\hline
%{\footnotesize $f_1(x) = (x^2 - 1)(x^2 + 1)$} & \cellcolor{red!100!green!15}18.4 & \cellcolor{red!66!green!15}15.7 & \cellcolor{red!10!green!15}11.3 & \cellcolor{red!5!green!15}11.0 & \cellcolor{red!0!green!15}10.5 & \cellcolor{red!100!green!15}25 & \cellcolor{red!77!green!15}20 & \cellcolor{red!0!green!15}0 & \cellcolor{red!36!green!15}9 & \cellcolor{red!38!green!15}10 & \cellcolor{red!100!green!15}1.5 & \cellcolor{red!66!green!15}1.29 & \cellcolor{red!19!green!15}1.0 & \cellcolor{red!6!green!15}0.92 & \cellcolor{red!0!green!15}0.89 \\
%{\footnotesize $f_2(x) = x^3 - 1$} & \cellcolor{red!100!green!15}15.5 & \cellcolor{red!69!green!15}13.3 & \cellcolor{red!10!green!15}9.1 & \cellcolor{red!10!green!15}9.1 & \cellcolor{red!0!green!15}8.4 & \cellcolor{red!100!green!15}8 & \cellcolor{red!53!green!15}4 & \cellcolor{red!0!green!15}0 & \cellcolor{red!16!green!15}1 & \cellcolor{red!14!green!15}1 & \cellcolor{red!100!green!15}1.55 & \cellcolor{red!67!green!15}1.35 & \cellcolor{red!11!green!15}1.0 & \cellcolor{red!1!green!15}0.94 & \cellcolor{red!0!green!15}0.93 \\
%{\footnotesize $f_3(x) = x^{12} - 1$} & \cellcolor{red!100!green!15}18.5 & \cellcolor{red!68!green!15}16.3 & \cellcolor{red!70!green!15}16.4 & \cellcolor{red!16!green!15}12.7 & \cellcolor{red!0!green!15}11.5 & \cellcolor{red!100!green!15}56 & \cellcolor{red!69!green!15}44 & \cellcolor{red!0!green!15}16 & \cellcolor{red!42!green!15}33 & \cellcolor{red!46!green!15}34 & \cellcolor{red!100!green!15}1.11 & \cellcolor{red!60!green!15}0.93 & \cellcolor{red!75!green!15}1.0 & \cellcolor{red!13!green!15}0.73 & \cellcolor{red!0!green!15}0.67 \\
%{\footnotesize $f_4(x) = (x^2 - 4)(x + 1.5)(x - 0.5)$} & \cellcolor{red!100!green!15}12.6 & \cellcolor{red!64!green!15}10.4 & \cellcolor{red!25!green!15}8.0 & \cellcolor{red!16!green!15}7.4 & \cellcolor{red!0!green!15}6.4 & \cellcolor{red!69!green!15}2 & \cellcolor{red!100!green!15}3 & \cellcolor{red!0!green!15}0 & \cellcolor{red!6!green!15}0 & \cellcolor{red!4!green!15}0 & \cellcolor{red!100!green!15}1.5 & \cellcolor{red!67!green!15}1.27 & \cellcolor{red!30!green!15}1.0 & \cellcolor{red!15!green!15}0.89 & \cellcolor{red!0!green!15}0.79 \\
%{\footnotesize $f_5(x) =(x+2)(x+1.5)^2 (x-0.5)(x-2)$} & \cellcolor{red!10!green!15}12.1 & \cellcolor{red!0!green!15}10.3 & \cellcolor{red!100!green!15}28.9 & \cellcolor{red!82!green!15}25.6 & \cellcolor{red!64!green!15}22.2 & \cellcolor{red!100!green!15}58 & \cellcolor{red!98!green!15}57 & \cellcolor{red!6!green!15}4 & \cellcolor{red!1!green!15}1 & \cellcolor{red!0!green!15}1 & \cellcolor{red!11!green!15}0.42 & \cellcolor{red!0!green!15}0.35 & \cellcolor{red!100!green!15}1.0 & \cellcolor{red!77!green!15}0.85 & \cellcolor{red!63!green!15}0.76 \\
%{\footnotesize $f_6(x) = \sin(x)$} & \cellcolor{red!100!green!15}9.7 & \cellcolor{red!53!green!15}7.7 & \cellcolor{red!26!green!15}6.6 & \cellcolor{red!11!green!15}6.0 & \cellcolor{red!0!green!15}5.5 & \cellcolor{red!77!green!15}13 & \cellcolor{red!100!green!15}16 & \cellcolor{red!0!green!15}0 & \cellcolor{red!28!green!15}5 & \cellcolor{red!46!green!15}8 & \cellcolor{red!100!green!15}1.42 & \cellcolor{red!46!green!15}1.09 & \cellcolor{red!31!green!15}1.0 & \cellcolor{red!9!green!15}0.87 & \cellcolor{red!0!green!15}0.82 \\
%{\footnotesize $f_7(x) = (x - 1)^3 + 4(x-1)^2 - 10$} & \cellcolor{red!100!green!15}17.9 & \cellcolor{red!64!green!15}14.5 & \cellcolor{red!13!green!15}9.7 & \cellcolor{red!7!green!15}9.1 & \cellcolor{red!0!green!15}8.4 & \cellcolor{red!100!green!15}3 & \cellcolor{red!93!green!15}3 & \cellcolor{red!0!green!15}0 & \cellcolor{red!2!green!15}0 & \cellcolor{red!1!green!15}0 & \cellcolor{red!100!green!15}1.74 & \cellcolor{red!67!green!15}1.44 & \cellcolor{red!18!green!15}1.0 & \cellcolor{red!9!green!15}0.92 & \cellcolor{red!0!green!15}0.83 \\
%{\footnotesize $f_8(x) = \sin(x-14/10)^2 - (x - 14/10)^2 + 1$} & \cellcolor{red!100!green!15}11.3 & \cellcolor{red!60!green!15}9.4 & \cellcolor{red!50!green!15}8.9 & \cellcolor{red!22!green!15}7.5 & \cellcolor{red!0!green!15}6.5 & \cellcolor{red!98!green!15}40 & \cellcolor{red!100!green!15}41 & \cellcolor{red!0!green!15}29 & \cellcolor{red!56!green!15}36 & \cellcolor{red!57!green!15}36 & \cellcolor{red!100!green!15}1.25 & \cellcolor{red!56!green!15}1.04 & \cellcolor{red!49!green!15}1.0 & \cellcolor{red!20!green!15}0.86 & \cellcolor{red!0!green!15}0.76 \\
%{\footnotesize $f_9(x) = x^2 - e^x - 3x + 2$} & \cellcolor{red!100!green!15}8.1 & \cellcolor{red!67!green!15}7.1 & \cellcolor{red!40!green!15}6.2 & \cellcolor{red!28!green!15}5.8 & \cellcolor{red!0!green!15}5.0 & \cellcolor{red!100!green!15}3 & \cellcolor{red!91!green!15}3 & \cellcolor{red!0!green!15}0 & \cellcolor{red!39!green!15}1 & \cellcolor{red!54!green!15}2 & \cellcolor{red!100!green!15}1.2 & \cellcolor{red!82!green!15}1.13 & \cellcolor{red!52!green!15}1.0 & \cellcolor{red!34!green!15}0.93 & \cellcolor{red!0!green!15}0.79 \\
%{\footnotesize $f_{10}(x) = \cos(x-3/4) - x + 3/4$} & \cellcolor{red!100!green!15}10.8 & \cellcolor{red!55!green!15}8.8 & \cellcolor{red!51!green!15}8.6 & \cellcolor{red!17!green!15}7.1 & \cellcolor{red!0!green!15}6.3 & \cellcolor{red!100!green!15}39 & \cellcolor{red!94!green!15}37 & \cellcolor{red!0!green!15}7 & \cellcolor{red!54!green!15}25 & \cellcolor{red!66!green!15}28 & \cellcolor{red!100!green!15}1.23 & \cellcolor{red!48!green!15}0.97 & \cellcolor{red!55!green!15}1.0 & \cellcolor{red!15!green!15}0.8 & \cellcolor{red!0!green!15}0.72 \\
%{\footnotesize $f_{11}(x) = (x + 1)^3 - 1$} & \cellcolor{red!100!green!15}15.1 & \cellcolor{red!66!green!15}12.7 & \cellcolor{red!13!green!15}9.0 & \cellcolor{red!11!green!15}8.9 & \cellcolor{red!0!green!15}8.1 & \cellcolor{red!100!green!15}7 & \cellcolor{red!50!green!15}4 & \cellcolor{red!0!green!15}0 & \cellcolor{red!15!green!15}1 & \cellcolor{red!14!green!15}1 & \cellcolor{red!100!green!15}1.5 & \cellcolor{red!67!green!15}1.29 & \cellcolor{red!23!green!15}1.0 & \cellcolor{red!17!green!15}0.96 & \cellcolor{red!0!green!15}0.85 \\
%{\footnotesize $f_{12}(x) = (x-2)^3 - 10$} & \cellcolor{red!100!green!15}17.5 & \cellcolor{red!67!green!15}14.7 & \cellcolor{red!4!green!15}9.3 & \cellcolor{red!10!green!15}9.8 & \cellcolor{red!0!green!15}8.9 & \cellcolor{red!100!green!15}13 & \cellcolor{red!58!green!15}8 & \cellcolor{red!0!green!15}0 & \cellcolor{red!20!green!15}3 & \cellcolor{red!12!green!15}2 & \cellcolor{red!100!green!15}1.84 & \cellcolor{red!66!green!15}1.54 & \cellcolor{red!4!green!15}1.0 & \cellcolor{red!5!green!15}1.01 & \cellcolor{red!0!green!15}0.96 \\
%{\footnotesize $f_{13}(x) = (x + 5/4)~  e^{(x + 5/4)^2} - \sin(x + 5/4)^2 + 3\cos(x + 5/4) + 5$} & \cellcolor{red!100!green!15}17.0 & \cellcolor{red!50!green!15}13.2 & \cellcolor{red!29!green!15}11.6 & \cellcolor{red!4!green!15}9.7 & \cellcolor{red!0!green!15}9.4 & \cellcolor{red!100!green!15}45 & \cellcolor{red!88!green!15}40 & \cellcolor{red!0!green!15}4 & \cellcolor{red!33!green!15}18 & \cellcolor{red!39!green!15}20 & \cellcolor{red!100!green!15}1.46 & \cellcolor{red!48!green!15}1.12 & \cellcolor{red!30!green!15}1.0 & \cellcolor{red!1!green!15}0.81 & \cellcolor{red!0!green!15}0.8 \\
%{\footnotesize $f_{14}(x) = (x + \sin(2/x)  x^2)$} & \cellcolor{red!100!green!15}15.5 & \cellcolor{red!66!green!15}13.5 & \cellcolor{red!23!green!15}10.9 & \cellcolor{red!0!green!15}9.5 & \cellcolor{red!13!green!15}10.3 & \cellcolor{red!100!green!15}65 & \cellcolor{red!65!green!15}43 & \cellcolor{red!0!green!15}1 & \cellcolor{red!18!green!15}12 & \cellcolor{red!40!green!15}26 & \cellcolor{red!100!green!15}1.41 & \cellcolor{red!65!green!15}1.22 & \cellcolor{red!25!green!15}1.0 & \cellcolor{red!0!green!15}0.86 & \cellcolor{red!41!green!15}1.08 \\
%\hline
%{\footnotesize $f(x) = (x^3 - 1)*e^{sin(z)/100}$} & \cellcolor{red!100!green!15}11.7 & \cellcolor{red!59!green!15}9.6 & \cellcolor{red!42!green!15}8.7 & \cellcolor{red!20!green!15}7.5 & \cellcolor{red!0!green!15}6.5 & \cellcolor{red!100!green!15}26 & \cellcolor{red!94!green!15}25 & \cellcolor{red!0!green!15}4 & \cellcolor{red!41!green!15}13 & \cellcolor{red!56!green!15}16 & \cellcolor{red!100!green!15}1.35 & \cellcolor{red!37!green!15}0.88 & \cellcolor{red!53!green!15}1.0 & \cellcolor{red!11!green!15}0.69 & \cellcolor{red!0!green!15}0.61 \\

==> table_2.tex <==
{\setlength\tabcolsep{0.1pt}%
\begin{tabular}{p{5.5cm}|>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}|>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}|>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}|>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}}
    \hline
{\multirow{2}{*}{Functions}}  &   \multicolumn{3}{c|}{Iter. number} &   \multicolumn{3}{c|}{Conv. percentage} &   \multicolumn{3}{c|}{Comp. time} & \multicolumn{3}{c}{Conv. order}  \\
    \cline{2-13}
& {\small$\beta=0$} & {\small$\beta=1$} & {\small$\beta_n$} & {\small$\beta=0$} & {\small$\beta=1$} & {\small$\beta_n$} & {\small$\beta=0$} & {\small$\beta=1$} & {\small$\beta_n$} & {\small$\beta=0$} & {\small$\beta=1$} & {\small$\beta_n$} \\
    \hline
{\footnotesize $f_1(x) = (x^2 - 1)(x^2 + 1)$}  & 11.3  & 10.5 & \hfil \bf{7.9} & \bf{100} & \hfil 90 & \bf{100}  & 1.0 & \bf{0.89} & 1.02 & 2.00 & 2.99 & \bf{4.08}  \\
\hline 
{\footnotesize $f_2(x) = x^3 - 1$}  & \hfil 9.1 & \hfil 8.4 & \hfil \bf{6.5} & \bf{100} & \hfil 99 & \bf{100} & 1.0 & \bf{0.93} & 1.07 & 2.00 & 3.01 & \bf{4.14} \\
\hline
{\footnotesize $f_3(x) = x^{12} - 1$}  & 16.4 & \bf{11.5} & 12.8 & \hfil 84 & \hfil 66 & \hfil \bf{87} & 1.0 & \bf{0.67} & 1.26 & 2.00 & 2.92 & \bf{4.17} \\
\hline
{\footnotesize $f_4(x) = (x^2 - 4)(x + 1.5)(x - 0.5)$}  & \hfil 8.0 & \hfil 6.4 & \hfil \bf{5.4} & \bf{100} & \bf{100} & \bf{100} & 1.0 & \bf{0.79} & 1.07 & 1.99 & 2.94 & \bf{3.95} \\
\hline
{\footnotesize $f_5(x) =(x+2)(x+1.5)^2 (x-0.5)(x-2)$}  & 28.9 & 22.2 & \bf{18.6} & \hfil 96 & \hfil 99 & \bf{100} & 1.0 & \bf{0.76} & 1.17 & 0.99 & \bf{1.00} & \bf{1.00} \\
\hline
{\footnotesize $f_6(x) = \sin(x)$}  & \hfil 6.6 & \hfil 5.5 & \hfil \bf{5.0} & \bf{100} & \hfil 92 & \hfil 99 & 1.0 & \bf{0.82} & 1.18 & 3.00 & 4.97 & \bf{6.85} \\
\hline 
{\footnotesize $f_7(x) = (x - 1)^3 + 4(x-1)^2 - 10$}  & \hfil 9.7 & \hfil 8.4 & \hfil \bf{7.3} & \bf{100} & \bf{100} & \bf{100} & 1.0 & \bf{0.83} & 1.44 & 2.00 & 3.02 & \bf{4.36} \\
\hline
{\footnotesize $f_8(x) = \sin(x-14/10)^2 - (x - 14/10)^2 + 1$}  & \hfil 8.9 & \hfil 6.5 & \hfil \bf{6.1} & \hfil 71 & \hfil 64 & \hfil \bf{73} & 1.0 & \bf{0.76} & 1.27 & 2.00 & \bf{2.98} & 2.58 \\
\hline
{\footnotesize $f_9(x) = x^2 - e^x - 3x + 2$}  & \hfil 6.2 & \hfil 5.0 & \hfil \bf{4.2} & \bf{100} & 98 & \bf{100} & 1.0 & \bf{0.79} & 0.99 & 2.00 & 3.09 & \bf{4.25} \\
\hline
{\footnotesize $f_{10}(x) = \cos(x-3/4) - x + 3/4$}  & \hfil 8.6 & \hfil \bf{6.3} & \hfil \bf{6.3} & \hfil \bf{93} & \hfil 72 & \hfil \bf{93} & 1.0 & \bf{0.72} & 1.17 & 2.00 & 3.02 & \bf{3.89} \\
\hline
{\footnotesize $f_{11}(x) = (x + 1)^3 - 1$}  & \hfil 9.0 & \hfil 8.1 & \hfil \bf{6.3} & \bf{100} & \hfil 99 & \bf{100} & 1.0 & \bf{0.85} & 1.23 & 2.00 & 2.93 & \bf{4.08} \\
\hline
{\footnotesize $f_{12}(x) = (x-2)^3 - 10$}  & \hfil 9.3 & \hfil 8.9 & \hfil \bf{7.0} & \bf{100} & \hfil 98 & \bf{100} & 1.0 & \bf{0.96} & 1.34 & 2.00 & 2.99 & \bf{3.92} \\
\hline
{\footnotesize $f_{13}(x) = (x + 5/4) e^{(x + 5/4)^2} - \sin(x + 5/4)^2 + 3\cos(x + 5/4) + 5$}  & 11.6 & \hfil 9.4 & \hfil \bf{8.5} & \hfil 96 & \hfil 80 & \hfil \bf{97} & 1.0 & \bf{0.80} & 1.34 & 2.00 & 3.02 & \bf{3.64} \\
\hline
{\footnotesize $f_{14}(x) = x + \sin(2/x)  x^2$}  & 10.9 & 10.3 & \hfil \bf{8.0} & \hfil \bf{99} & \hfil 74 & \hfil 81 & \bf{1.0} & 1.08 & 1.28 & 2.00 & 2.99 & \bf{3.99} \\
\hline
\end{tabular}
}
%\begin{tabular}{p{6cm} ddd | ddd |ddd | d}
% & \multicolumn{3}{c}{Mean it. per pt} & \multicolumn{3}{c}{Non conv. (\%)} &\multicolumn{3}{c}{T per pt } & \multicolumn{1}{c}{$q_{ann}$}\\
% & \multicolumn{3}{c}{$\beta$} & \multicolumn{3}{c}{$\beta$} &\multicolumn{3}{c}{$\beta$} &\\    
% & 0 & 1 & ann.  &  0 & 1 & ann.  & 0 & 1 & ann.  \\
%\hline
%{\footnotesize $f_1(x) = (x^2 - 1)(x^2 + 1)$}  & \cellcolor{red!100!green!15}11.3 & \cellcolor{red!78!green!15}10.5 & \cellcolor{red!0!green!15}7.9 & \cellcolor{red!2!green!15}0 & \cellcolor{red!100!green!15}10 & \cellcolor{red!0!green!15}0 & \cellcolor{red!83!green!15}1.0 & \cellcolor{red!0!green!15}0.89 & \cellcolor{red!100!green!15}1.02 & 4.08 \\
%{\footnotesize $f_2(x) = x^3 - 1$}  & \cellcolor{red!100!green!15}9.1 & \cellcolor{red!73!green!15}8.4 & \cellcolor{red!0!green!15}6.5 & \cellcolor{red!0!green!15}0 & \cellcolor{red!100!green!15}1 & \cellcolor{red!0!green!15}0 & \cellcolor{red!49!green!15}1.0 & \cellcolor{red!0!green!15}0.93 & \cellcolor{red!100!green!15}1.07 & 4.14 \\
%{\footnotesize $f_3(x) = x^{12} - 1$}  & \cellcolor{red!100!green!15}16.4 & \cellcolor{red!0!green!15}11.5 & \cellcolor{red!26!green!15}12.8 & \cellcolor{red!14!green!15}16 & \cellcolor{red!100!green!15}34 & \cellcolor{red!0!green!15}13 & \cellcolor{red!56!green!15}1.0 & \cellcolor{red!0!green!15}0.67 & \cellcolor{red!100!green!15}1.26 & 4.17 \\
%{\footnotesize $f_4(x) = (x^2 - 4)(x + 1.5)(x - 0.5)$}  & \cellcolor{red!100!green!15}8.0 & \cellcolor{red!40!green!15}6.4 & \cellcolor{red!0!green!15}5.4 & \cellcolor{red!0!green!15}0 & \cellcolor{red!100!green!15}0 & \cellcolor{red!0!green!15}0 & \cellcolor{red!74!green!15}1.0 & \cellcolor{red!0!green!15}0.79 & \cellcolor{red!100!green!15}1.07 & 3.95 \\
%{\footnotesize $f_5(x) =(x+2)(x+1.5)^2 (x-0.5)(x-2)$}  & \cellcolor{red!100!green!15}28.9 & \cellcolor{red!35!green!15}22.2 & \cellcolor{red!0!green!15}18.6 & \cellcolor{red!100!green!15}4 & \cellcolor{red!15!green!15}1 & \cellcolor{red!0!green!15}0 & \cellcolor{red!59!green!15}1.0 & \cellcolor{red!0!green!15}0.76 & \cellcolor{red!100!green!15}1.17 & 1.0 \\
%{\footnotesize $f_6(x) = \sin(x)$}  & \cellcolor{red!100!green!15}6.6 & \cellcolor{red!33!green!15}5.5 & \cellcolor{red!0!green!15}5.0 & \cellcolor{red!0!green!15}0 & \cellcolor{red!100!green!15}8 & \cellcolor{red!3!green!15}1 & \cellcolor{red!50!green!15}1.0 & \cellcolor{red!0!green!15}0.82 & \cellcolor{red!100!green!15}1.18 & 6.85 \\
%{\footnotesize $f_7(x) = (x - 1)^3 + 4(x-1)^2 - 10$}  & \cellcolor{red!100!green!15}9.7 & \cellcolor{red!46!green!15}8.4 & \cellcolor{red!0!green!15}7.3 & \cellcolor{red!0!green!15}0 & \cellcolor{red!100!green!15}0 & \cellcolor{red!0!green!15}0 & \cellcolor{red!27!green!15}1.0 & \cellcolor{red!0!green!15}0.83 & \cellcolor{red!100!green!15}1.44 & 4.36 \\
%{\footnotesize $f_8(x) = \sin(x-14/10)^2 - (x - 14/10)^2 + 1$}  & \cellcolor{red!100!green!15}8.9 & \cellcolor{red!13!green!15}6.5 & \cellcolor{red!0!green!15}6.1 & \cellcolor{red!26!green!15}29 & \cellcolor{red!100!green!15}36 & \cellcolor{red!0!green!15}27 & \cellcolor{red!47!green!15}1.0 & \cellcolor{red!0!green!15}0.76 & \cellcolor{red!100!green!15}1.27 & 2.58 \\
%{\footnotesize $f_9(x) = x^2 - e^x - 3x + 2$}  & \cellcolor{red!100!green!15}6.2 & \cellcolor{red!37!green!15}5.0 & \cellcolor{red!0!green!15}4.2 & \cellcolor{red!0!green!15}0 & \cellcolor{red!100!green!15}2 & \cellcolor{red!0!green!15}0 & \cellcolor{red!100!green!15}1.0 & \cellcolor{red!0!green!15}0.79 & \cellcolor{red!96!green!15}0.99 & 4.25 \\
%{\footnotesize $f_{10}(x) = \cos(x-3/4) - x + 3/4$}  & \cellcolor{red!100!green!15}8.6 & \cellcolor{red!3!green!15}6.3 & \cellcolor{red!0!green!15}6.3 & \cellcolor{red!0!green!15}7 & \cellcolor{red!100!green!15}28 & \cellcolor{red!0!green!15}7 & \cellcolor{red!63!green!15}1.0 & \cellcolor{red!0!green!15}0.72 & \cellcolor{red!100!green!15}1.17 & 3.89 \\
%{\footnotesize $f_{11}(x) = (x + 1)^3 - 1$}  & \cellcolor{red!100!green!15}9.0 & \cellcolor{red!66!green!15}8.1 & \cellcolor{red!0!green!15}6.3 & \cellcolor{red!0!green!15}0 & \cellcolor{red!100!green!15}1 & \cellcolor{red!0!green!15}0 & \cellcolor{red!40!green!15}1.0 & \cellcolor{red!0!green!15}0.85 & \cellcolor{red!100!green!15}1.23 & 4.08 \\
%{\footnotesize $f_{12}(x) = (x-2)^3 - 10$}  & \cellcolor{red!100!green!15}9.3 & \cellcolor{red!84!green!15}8.9 & \cellcolor{red!0!green!15}7.0 & \cellcolor{red!0!green!15}0 & \cellcolor{red!100!green!15}2 & \cellcolor{red!0!green!15}0 & \cellcolor{red!10!green!15}1.0 & \cellcolor{red!0!green!15}0.96 & \cellcolor{red!100!green!15}1.34 & 3.92 \\
%{\footnotesize $f_{13}(x) = (x + 5/4)~  e^{(x + 5/4)^2} - \sin(x + 5/4)^2 + 3\cos(x + 5/4) + 5$}  & \cellcolor{red!100!green!15}11.6 & \cellcolor{red!29!green!15}9.4 & \cellcolor{red!0!green!15}8.5 & \cellcolor{red!7!green!15}4 & \cellcolor{red!100!green!15}20 & \cellcolor{red!0!green!15}3 & \cellcolor{red!37!green!15}1.0 & \cellcolor{red!0!green!15}0.8 & \cellcolor{red!100!green!15}1.34 & 3.64 \\
%{\footnotesize $f_{14}(x) = (x + \sin(2/x)  x^2)$}  & \cellcolor{red!100!green!15}10.9 & \cellcolor{red!80!green!15}10.3 & \cellcolor{red!0!green!15}8.0 & \cellcolor{red!0!green!15}1 & \cellcolor{red!100!green!15}26 & \cellcolor{red!73!green!15}19 & \cellcolor{red!0!green!15}1.0 & \cellcolor{red!31!green!15}1.08 & \cellcolor{red!100!green!15}1.28 & 3.99 \\
%\end{tabular}
%}
